Depth3DLane: Monocular 3D Lane Detection via Depth Prior Distillation

Monocular 3D lane detection is challenging due to the difficulty in capturing depth information from single-camera images. A common strategy involves transforming front-view (FV) images into bird's-eye-view (BEV) space through inverse perspective mapping (IPM), facilitating lane detection using BEV features. However, IPM's flat-ground assumption and loss of contextual information lead to inaccuracies in reconstructing 3D information, especially height. In this paper, we introduce a BEV-based framework to address these limitations and improve 3D lane detection accuracy. Our approach incorporates a Hierarchical Depth-Aware Head that provides multi-scale depth features, mitigating the flat-ground assumption by enhancing spatial awareness across varying depths. Additionally, we leverage Depth Prior Distillation to transfer semantic depth knowledge from a teacher model, capturing richer structural and contextual information for complex lane structures. To further refine lane continuity and ensure smooth lane reconstruction, we introduce a Conditional Random Field module that enforces spatial coherence in lane predictions. Extensive experiments validate that our method achieves state-of-the-art performance in terms of z-axis error and outperforms other methods in the field in overall performance. The code is released at: https://anonymous.4open.science/r/Depth3DLane-DCDD.

==> tabs/apollo_new.tex <==
\begin{table*}
\setlength{\tabcolsep}{0.005pt}
\begin{tabular}{@{}c|ccccc|ccccc@{}}
        \Xhline{1.5pt}
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Balanced Scene}} & \multicolumn{5}{c}{\textbf{Rarely Observed}} \\
        \cline{2-11}
        & \textbf{F1(\%)}\uparrow & \textbf{x-Err/N(m)}\downarrow & \textbf{x-Err/F(m)}\downarrow & \textbf{z-Err/N(m)}\downarrow & \textbf{z-Err/F(m)}\downarrow & \textbf{F1(\%)}\uparrow & \textbf{x-Err/N(m)}\downarrow & \textbf{x-Err/F(m)}\downarrow & \textbf{z-Err/N(m)}\downarrow & \textbf{z-Err/F(m)}\downarrow \\
        \hline
        \hline
        PersFormer~\cite{chen2022persformer} & 92.9 & 0.054 & 0.356 & 0.010 & 0.234 & 87.5 & \textbf{0.107} & 0.782 & 0.024 & 0.602 \\
        Anchor3DLane~\cite{huang2023anchor3dlane} & 95.6 & 0.052 & 0.306 & 0.015 & 0.223 & 94.4 & 0.094 & 0.693 & 0.027 & 0.579 \\
        BEV-LaneDet~\cite{wang2023bev} & 98.7 & \textbf{0.016} & \textbf{0.242} & 0.020 & 0.216 & 99.1 & 0.031 & 0.594 & 0.040 & 0.556 \\
        LATR~\cite{luo2023latr} & 96.8 & 0.022 & 0.253 & \textbf{0.007} & 0.202 & 96.1 & 0.050 & 0.600 & \textbf{0.015} & 0.532 \\
        LaneCPP~\cite{Pittner2024LaneCPP} & 97.4 & 0.030 & 0.277 & 0.011 & 0.206 & 96.2 & 0.073 & 0.651 & 0.023 & 0.543 \\
        DV-3DLane~\cite{Luo2024DV3DLane} & 96.4 & 0.046 & 0.299 & 0.016 & 0.213 & 95.6 & 0.071 & 0.664 & 0.025 & 0.568 \\ 
        \hline
        \rowcolor{gray!40}
        Depth3DLane (Ours) & \textbf{98.9} & 0.027 & 0.303 & 0.012 & \textbf{0.201} & \textbf{99.2} & 0.026 & \textbf{0.547} & 0.032 & \textbf{0.524} \\        
        \Xhline{1.5pt}
    \end{tabular}
    \end{table*}

==> tabs/compare_apollo.tex <==
\begin{table}
    \centering
    \renewcommand{\arraystretch}{1} % Adjust row height
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{@{}c|c|ccc@{}}
        \toprule
        \textbf{Methods} & \textbf{\#param.} & \textbf{F1-Score(\%)} & \textbf{AP} & \textbf{FPS} \\
        \midrule
        LATR-lite\cite{luo2023latr} & ResNet-50 & 61.5 & 91.9 & 23.5 \\
        LATR\cite{luo2023latr} & ResNet-50 & \textbf{61.9} & \textbf{92.0} & 15.2 \\
        Depth3DLane & ResNet-18 & 61.5 & 91.7 & \textbf{88.0} \\
        \bottomrule
    \end{tabular}}
    \caption{Model performance (F1) vs Execution Speed (FPS) on OpenLane\cite{chen2022persformer} Dataset}
    \label{tab:scale_combinations}
\end{table}

==> tabs/compare_openlane.tex <==
% \begin{table}[htbp]
%     \centering
%     \renewcommand{\arraystretch}{1} % Adjust row height
%     \setlength{\tabcolsep}{1.2mm}{
%     \begin{tabular}{@{}c|c|c|c@{}}
%         \toprule
%         \textbf{Methods} & \textbf{Backbone} & \textbf{F1-Score(\%)} & \textbf{FPS} \\
%         \midrule
%         LATR-Lite & ResNet-50 & 61.5 & 23.5 \\
%         LATR & ResNet-50 & 61.9 & 15.2 \\
%          \rowcolor{gray!20} Depth3DLane & ResNet-34 & 61.5 & \textbf{88.0} \\
%          \rowcolor{gray!20} Depth3DLane & ResNet-50 & 62.7 & 74.6 \\
%          \rowcolor{gray!20} Depth3DLane & Swin-B & \textbf{64.5} & 56.2 \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Comparison of Model Performance (F1-Score, Cate Accuracy) and Execution Speed (FPS) on the OpenLane Dataset.}
%     \label{tab:scale_combinations}
% \end{table}


\begin{table}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|c|cc|c}
        \hline
        \multirow{2}{*}{\textbf{Methods}} 
          & \multirow{2}{*}{\textbf{Backbone}} 
          & \multicolumn{2}{c|}{\textbf{F1-Score (\%)}} 
          & \multirow{2}{*}{\textbf{FPS}} \\
        \cline{3-4}
        & 
          & \textbf{OpenLane} 
          & \textbf{ApolloSim} 
          & \\ 
        \hline
        LATR-Lite    & ResNet-50 & 61.5      & 96.5       & 23.5 \\
        LATR         & ResNet-50 & 61.9      & 96.8       & 15.2 \\
        Depth3DLane  & ResNet-34 & 61.5      & \textbf{98.9}      & \textbf{88.0} \\
        Depth3DLane  & ResNet-50 & 62.7      & -    & 58.2 \\
        Depth3DLane  & Swin-B    & \textbf{64.5} & - & 45.7 \\
        \hline
    \end{tabular}
    }
    \caption{Comparison of Model Performance F1-Score and Execution Speed (FPS) on the OpenLane and ApolloSim Dataset.}
    \label{tab:scale_combinations}
\end{table}


% \begin{table}[htbp]
%   \centering
%   \renewcommand{\arraystretch}{1.2} % 行高
%   \setlength{\tabcolsep}{1.8mm}     % 列间距
%   \begin{tabular}{@{}c|c|cc|c@{}}
%     \toprule
%     \textbf{Methods} 
%       & \textbf{Backbone} 
%       & \multicolumn{2}{c|}{\textbf{F1-Score (\%)}} 
%       & \textbf{FPS} \\
%     \cmidrule(lr){3-4}
%     % 下面这一行，第一、二、五列留空，只有 3–4 列放子标题
%       & 
%       & \textbf{Apollo} 
%       & \textbf{OpenLane} 
%       &  \\
%     \midrule
%     LATR-Lite    & ResNet-50 & 61.5 & 58.2 & 23.5 \\
%     LATR         & ResNet-50 & 61.9 & 59.7 & 15.2 \\
%     \rowcolor{gray!20}
%     Depth3DLane  & ResNet-34 & 61.5 & 60.1 & \textbf{88.0} \\
%     \rowcolor{gray!20}
%     Depth3DLane  & ResNet-50 & 62.7 & 61.3 & 74.6 \\
%     \rowcolor{gray!20}
%     Depth3DLane  & Swin-B    & \textbf{64.5} & 62.9 & 56.2 \\
%     \bottomrule
%   \end{tabular}
%   \caption{在 Apollo 与 OpenLane 两个数据集上的模型性能及推理速度对比}
%   \label{tab:two_datasets}
% \end{table}


==> tabs/depth_head.tex <==
\begin{table}
    \centering
    \renewcommand{\arraystretch}{1} % 调整行高
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{@{}c|cc|ccc@{}}
        \toprule
        \textbf{Depth Head} & \textbf{ssim} & \textbf{silog} & \textbf{F-Score} & \textbf{z-Err/C(m)} & \textbf{z-Err/F(m)} \\
        \midrule
        - & - & - & 58.4 & 0.130 & 0.606 \\
        \checkmark & \checkmark & & 58.6 & 0.142 & 0.258 \\
        \checkmark &  & \checkmark & 60.1 & 0.122 & 0.140 \\
        \checkmark & \checkmark & \checkmark & \textbf{60.2} & 0\textbf{.115} & \textbf{0.135} \\
        \bottomrule
    \end{tabular}}
    \caption{Ablation studies on the Depth Head module with different loss function. Only the Depth Head is enabled, while the CRF and Distillation modules are disabled.}
    \label{tab:depth_head}
\end{table}


==> tabs/distillation.tex <==
\begin{table}
    \centering
    \renewcommand{\arraystretch}{1} % 调整行高
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{@{}c|cc|ccc@{}}
        \toprule
        \textbf{Distillation} & \textbf{MSE} & \textbf{cos} & \textbf{F-Score} & \textbf{z-Err/C(m)} & \textbf{z-Err/F(m)} \\
        \midrule
        - & - & - & 58.4 & 0.130 & 0.606 \\
        \checkmark & \checkmark & & 59.4& 0.127& 0.142\\
        \checkmark &  & \checkmark & 57.9& 0.134& \textbf{0.136}\\
        \checkmark & \checkmark & \checkmark & \textbf{59.7}& \textbf{0.125}& 0.137\\
        \bottomrule
    \end{tabular}}
    \caption{Ablation studies on the Distillation module with different loss function. Only the Distillation module is enabled, while the Depth Head and CRF modules are disabled.}
    \label{tab:distillation}
\end{table}

